Deep Speech Synthesis from Articulatory Representations

In the articulatory synthesis task, speech is synthesized from input features containing information about the physical behavior of the human vocal tract. This task provides a promising direction for speech synthesis research, as the articulatory space is compact, smooth, and interpretable. Current works have highlighted the potential for deep learning models to perform articulatory synthesis. However, it remains unclear whether these models can achieve the efficiency and fidelity of the human speech production system. To help bridge this gap, we propose a time-domain articulatory synthesis methodology and demonstrate its efficacy with both electromagnetic articulography (EMA) and synthetic articulatory feature inputs. Our model is computationally efficient and achieves a transcription word error rate (WER) of 18.5% for the EMA-to-speech task, yielding an improvement of 11.6% compared to prior work. Through interpolation experiments, we also highlight the generalizability and interpretability of our approach.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> peter_art_22_arxiv <==
% Generated by IEEEtran.bst, version: 1.13 (2008/09/30)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Wang2017Tacotron}
Y.~Wang \emph{et~al.}, ``Tacotron: Towards end-to-end speech synthesis,'' in
  \emph{Interspeech}, 2017.

\bibitem{hayashi2021espnet2}
T.~Hayashi \emph{et~al.}, ``Espnet2-tts: Extending the edge of tts research,''
  \emph{arXiv preprint arXiv:2110.07840}, 2021.

\bibitem{prenger2019waveglow}
R.~Prenger, R.~Valle, and B.~Catanzaro, ``Waveglow: A flow-based generative
  network for speech synthesis,'' in \emph{ICASSP}, 2019.

\bibitem{tjandra2019speechtranslation}
A.~Tjandra, S.~Sakti, and S.~Nakamura, ``Speech-to-speech translation between
  untranscribed unknown languages,'' in \emph{ASRU}, 2019, pp. 593--600.

\bibitem{jia2019speechtranslation}
Y.~Jia \emph{et~al.}, ``Direct speech-to-speech translation with a
  sequence-to-sequence model,'' in \emph{Interspeech}, 2019.

\bibitem{inaguma2020espnetspeechtranslation}
H.~Inaguma \emph{et~al.}, ``{ESP}net-{ST}: All-in-one speech translation
  toolkit,'' in \emph{ACL}, 2020.

\bibitem{polyak21facebookresynthesis}
A.~Polyak \emph{et~al.}, ``{Speech Resynthesis from Discrete Disentangled
  Self-Supervised Representations},'' in \emph{Interspeech}, 2021.

\bibitem{wu2021privacy}
P.~Wu \emph{et~al.}, ``Understanding the tradeoffs in client-side privacy for
  downstream speech tasks,'' in \emph{APSIPA ASC}, 2021.

\bibitem{sisman2020overview}
B.~Sisman \emph{et~al.}, ``An overview of voice conversion and its challenges:
  From statistical modeling to deep learning,'' \emph{TASLP}, 2020.

\bibitem{anumanchipalli2019speech}
G.~K. Anumanchipalli, J.~Chartier, and E.~F. Chang, ``Speech synthesis from
  neural decoding of spoken sentences,'' \emph{Nature}, vol. 568, no. 7753, pp.
  493--498, 2019.

\bibitem{yu2019durianmultimodalsynthesis}
C.~Yu \emph{et~al.}, ``Durian: Duration informed attention network for
  multimodal synthesis,'' \emph{arXiv preprint arXiv:1909.01700}, 2019.

\bibitem{gaddy-klein-2021-improved}
D.~Gaddy and D.~Klein, ``An improved model for voicing silent speech,'' in
  \emph{ACL-IJCNLP}, 2021.

\bibitem{karmel2019speechsynthesisforblind}
A.~Karmel \emph{et~al.}, ``Iot based assistive device for deaf, dumb and blind
  people,'' \emph{ICRTAC}, 2019.

\bibitem{angrick2019ecogbraintospeech}
M.~Angrick \emph{et~al.}, ``Speech synthesis from ecog using densely connected
  3d convolutional neural networks,'' \emph{Journal of neural engineering},
  vol.~16, no.~3, p. 036019, 2019.

\bibitem{jia2021translatotron}
Y.~Jia \emph{et~al.}, ``Translatotron 2: Robust direct speech-to-speech
  translation,'' \emph{arXiv preprint arXiv:2107.08661}, 2021.

\bibitem{Nekvinda2020multilingualtts}
T.~Nekvinda and O.~Dušek, ``{One Model, Many Languages: Meta-Learning for
  Multilingual Text-to-Speech},'' in \emph{Interspeech}, 2020.

\bibitem{zhang2019multilingualtts}
Y.~Zhang \emph{et~al.}, ``Learning to speak fluently in a foreign language:
  Multilingual speech synthesis and cross-language voice cloning,'' \emph{arXiv
  preprint arXiv:1907.04448}, 2019.

\bibitem{fant1991articulatorysynthesis}
G.~Fant, ``What can basic research contribute to speech synthesis?''
  \emph{Journal of Phonetics}, vol.~19, no.~1, pp. 75--90, 1991.

\bibitem{rubin1981articulatorysynthesis}
P.~Rubin, T.~Baer, and P.~Mermelstein, ``An articulatory synthesizer for
  perceptual research,'' \emph{The Journal of the Acoustical Society of
  America}, vol.~70, no.~2, pp. 321--328, 1981.

\bibitem{scully1990articulatorysynthesis}
C.~Scully, ``Articulatory synthesis,'' in \emph{Speech production and speech
  modelling}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 1990, pp.
  151--186.

\bibitem{jiachen2022gesture}
J.~Lian, A.~W. Black, L.~Goldstein, and G.~K. Anumanchipalli, ``Deep neural
  convolutive matrix factorization for articulatory representation
  decomposition,'' \emph{Interspeech}, 2022.

\bibitem{fant1995lfvocaltractmodal}
G.~Fant, ``The lf-model revisited. transformations and frequency domain
  analysis,'' \emph{Speech Trans. Lab. Q. Rep., Royal Inst. of Tech.
  Stockholm}, vol.~2, no.~3, p.~40, 1995.

\bibitem{iskarous2003haskinscasy}
K.~Iskarous \emph{et~al.}, ``Casy: The haskins configurable articulatory
  synthesizer,'' in \emph{International Congress of Phonetic Sciences}, 2003.

\bibitem{birkholz2013vtl}
P.~Birkholz, ``Modeling consonant-vowel coarticulation for articulatory speech
  synthesis,'' \emph{PloS one}, vol.~8, no.~4, p. e60603, 2013.

\bibitem{aryal2016datadrivendnn}
S.~Aryal and R.~Gutierrez-Osuna, ``Data driven articulatory synthesis with deep
  neural networks,'' \emph{Computer Speech \& Language}, vol.~36, pp. 260--273,
  2016.

\bibitem{bocquelet2014dnn}
F.~Bocquelet \emph{et~al.}, ``Robust articulatory speech synthesis using deep
  neural networks for bci applications,'' in \emph{Interspeech}, 2014.

\bibitem{chen2021ema2s}
Y.-W. Chen \emph{et~al.}, ``Ema2s: An end-to-end multimodal
  articulatory-to-speech system,'' in \emph{ISCAS}, 2021.

\bibitem{kong2020hifigan}
J.~Kong, J.~Kim, and J.~Bae, ``Hifi-gan: Generative adversarial networks for
  efficient and high fidelity speech synthesis,'' in \emph{NeurIPS}, 2020.

\bibitem{morrison2022cargan}
M.~Morrison \emph{et~al.}, ``Chunked autoregressive gan for conditional
  waveform synthesis,'' in \emph{Submitted to ICLR 2022}, April 2022.

\bibitem{badlani2021onettsalignment}
R.~Badlani \emph{et~al.}, ``One tts alignment to rule them all,'' \emph{arXiv
  preprint arXiv:2108.10447}, 2021.

\bibitem{kim2021vits}
J.~Kim, J.~Kong, and J.~Son, ``Conditional variational autoencoder with
  adversarial learning for end-to-end text-to-speech,'' in \emph{ICML}, 2021.

\bibitem{Elias2021ParallelTacotron2}
I.~Elias \emph{et~al.}, ``Parallel tacotron 2: A non-autoregressive neural tts
  model with differentiable duration modeling,'' \emph{ArXiv}, vol.
  abs/2103.14574, 2021.

\bibitem{nam2012procedure}
H.~Nam \emph{et~al.}, ``A procedure for estimating gestural scores from speech
  acoustics,'' \emph{The Journal of the Acoustical Society of America}, vol.
  132, no.~6, pp. 3980--3989, 2012.

\bibitem{richmond2011mngu0}
K.~Richmond, P.~Hoole, and S.~King, ``Announcing the electromagnetic
  articulography (day 1) subset of the mngu0 articulatory corpus,'' in
  \emph{Interspeech}, 08 2011, pp. 1505--1508.

\bibitem{taguchi2018articulatory}
F.~Taguchi and T.~Kaburagi, ``Articulatory-to-speech conversion using
  bi-directional long short-term memory.'' in \emph{Interspeech}, 2018, pp.
  2499--2503.

\bibitem{stone2020ema}
S.~Stone, P.~Schmidt, and P.~Birkholz, ``Prediction of voicing and the f0
  contour from electromagnetic articulography data for articulation-to-speech
  synthesis,'' in \emph{ICASSP}, 2020.

\bibitem{liu2018articulatory}
Z.-C. Liu, Z.-H. Ling, and L.-R. Dai, ``Articulatory-to-acoustic conversion
  using blstm-rnns with augmented input representation,'' \emph{Speech
  Communication}, vol.~99, pp. 161--172, 2018.

\bibitem{Csapo2020UltrasoundbasedAM}
T.~G. Csap'o \emph{et~al.}, ``Ultrasound-based articulatory-to-acoustic mapping
  with waveglow speech synthesis,'' in \emph{Interspeech}, 2020.

\bibitem{georges2020towards}
M.-A. Georges \emph{et~al.}, ``Towards an articulatory-driven neural vocoder
  for speech synthesis,'' in \emph{International Seminar on Speech Production},
  2020.

\bibitem{Vaswani2017attentiontransformer}
A.~Vaswani \emph{et~al.}, ``Attention is all you need,'' in \emph{NeurIPS},
  2017.

\bibitem{kim2018crepe}
J.~W. Kim \emph{et~al.}, ``Crepe: A convolutional representation for pitch
  estimation,'' in \emph{ICASSP}, 2018.

\bibitem{hagedorn11_interspeech}
C.~Hagedorn, M.~Proctor, and L.~Goldstein, ``{Automatic analysis of singleton
  and geminate consonant articulation using real-time magnetic resonance
  imaging},'' in \emph{Interspeech}, 2011.

\bibitem{lenzo2003kal}
K.~Lenzo and A.~Black, ``Diphone collection and synthesis,'' \emph{ICSLP},
  2000.

\bibitem{alfonso1982dynamics}
P.~J. Alfonso and T.~Baer, ``Dynamics of vowel articulation,'' \emph{Language
  and Speech}, vol.~25, no.~2, pp. 151--173, 1982.

\bibitem{pmlr-v80-wang18h}
Y.~Wang \emph{et~al.}, ``Style tokens: Unsupervised style modeling, control and
  transfer in end-to-end speech synthesis,'' in \emph{ICML}, 2018.

\bibitem{sun2020taco}
G.~Sun \emph{et~al.}, ``Fully-hierarchical fine-grained prosody modeling for
  interpretable speech synthesis,'' in \emph{ICASSP}, 2020.

\bibitem{black2019cmu_wilderness}
A.~W. Black, ``{CMU} wilderness multilingual speech dataset,'' in
  \emph{ICASSP}, 2019.

\bibitem{Hannun2014DeepSpeech}
A.~Y. Hannun \emph{et~al.}, ``Deep speech: Scaling up end-to-end speech
  recognition,'' \emph{ArXiv}, vol. abs/1412.5567, 2014.

\bibitem{baevski2020wav2vec2}
A.~Baevski \emph{et~al.}, ``Wav2vec 2.0: A framework for self-supervised
  learning of speech representations,'' in \emph{NeurIPS}, 2020.

\bibitem{speechbrain}
M.~Ravanelli \emph{et~al.}, ``{SpeechBrain}: A general-purpose speech
  toolkit,'' 2021, arXiv:2106.04624.

\bibitem{Bernard2021phonemizer}
M.~Bernard and H.~Titeux, ``Phonemizer: Text to phones transcription for
  multiple languages in python,'' \emph{Journal of Open Source Software},
  vol.~6, no.~68, p. 3958, 2021.

\bibitem{alwan2011plosivefricative}
A.~Alwan, J.~Jiang, and W.~Chen, ``Perception of place of articulation for
  plosives and fricatives in noise,'' \emph{Speech communication}, vol.~53,
  no.~2, pp. 195--209, 2011.

\bibitem{lim2021mri}
Y.~Lim \emph{et~al.}, ``A multispeaker dataset of raw and reconstructed speech
  production real-time mri video and 3d volumetric images,'' \emph{Scientific
  Data}, vol.~8, 07 2021.

\end{thebibliography}

